Score-based Generative Models for Photoacoustic Image Reconstruction with Rotation Consistency Constraints

Photoacoustic tomography (PAT) is a newly emerged imaging modality which enables both high optical contrast and acoustic depth of penetration. Reconstructing images of photoacoustic tomography from limited amount of senser data is among one of the major challenges in photoacoustic imaging. Previous works based on deep learning were trained in supervised fashion, which directly map the input partially known sensor data to the ground truth reconstructed from full field of view. Recently, score-based generative models played an increasingly significant role in generative modeling. Leveraging this probabilistic model, we proposed Rotation Consistency Constrained Score-based Generative Model (RCC-SGM), which recovers the PAT images by iterative sampling between Langevin dynamics and a constraint term utilizing the rotation consistency between the images and the measurements. Our proposed method can generalize to different measurement processes (32.29 PSNR with 16 measurements under random sampling, whereas 28.50 for supervised counterpart), while supervised methods need to train on specific inverse mappings.

==> contents/related_works.tex <==
\section{Related Works}\label{sec:related_works}

\paragraph{Supervised PAT reconstruction approaches} Hengrong Lan et al.~proposed Ki-GAN to generate images using a GAN with well-designed autoencoders~\cite{Lan2019KiGANKI}. Steven Guan et al.~proposed fully dense UNet which utilized skip connections to enhance UNet~\cite{Guan2019LimitedViewAS}. Hengrong Lan's companion work further proposed Y-Net to reconstruct PAT images combining both information from undersampled measurements and noisy images with a supervised CNN architecture~\cite{Lan2020YNetHD}.

\paragraph{Score-based generative model for medical inverse problems} Ajil Jalal et al.~proposed a sampling algorithm using gradient of likelihood to guide the annealed Langevin dynamics~\cite{Jalal2021RobustCS}. Besides, Hyungjin Chung et al.~proposed several improvements on score-based generative models, including utilizing different constrain terms~\cite{Chung2021ScorebasedDM,Chung2022ImprovingDM} and different modifications on sampling processes~\cite{Chung2021ComeCloserDiffuseFasterAC}. In addition, Yang Song et al.~demonstrated that by gradually mixing measurements, predicted images and sampling patterns, a sampling process can produce even higher quality recontructions with deep generative priors~\cite{Song2021SolvingIP}.
Xiangxi Meng et al.~designed a novel framework for multi-modal medical image completion which adopted a multi-in multi-out architecture~\cite{Meng2022ANU}.

